Towards Dynamic Message Passing on Graphs

Message passing plays a vital role in graph neural networks (GNNs) for effective feature learning. However, the over-reliance on input topology diminishes the efficacy of message passing and restricts the ability of GNNs. Despite efforts to mitigate the reliance, existing study encounters message-passing bottlenecks or high computational expense problems, which invokes the demands for flexible message passing with low complexity. In this paper, we propose a novel dynamic message-passing mechanism for GNNs. It projects graph nodes and learnable pseudo nodes into a common space with measurable spatial relations between them. With nodes moving in the space, their evolving relations facilitate flexible pathway construction for a dynamic message-passing process. Associating pseudo nodes to input graphs with their measured relations, graph nodes can communicate with each other intermediately through pseudo nodes under linear complexity. We further develop a GNN model named $\mathtt{\mathbf{N^2}}$ based on our dynamic message-passing mechanism. $\mathtt{\mathbf{N^2}}$ employs a single recurrent layer to recursively generate the displacements of nodes and construct optimal dynamic pathways. Evaluation on eighteen benchmarks demonstrates the superior performance of $\mathtt{\mathbf{N^2}}$ over popular GNNs. $\mathtt{\mathbf{N^2}}$ successfully scales to large-scale benchmarks and requires significantly fewer parameters for graph classification with the shared recurrent layer.

==> comp-tex/analysis-ablation.tex <==
\begin{table*}
    \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/num pnode.pdf}
        \vspace{-0.1in}
        \figcaption{\textbf{Ablation Studies on the Number of Pseudo-nodes ( $n_p$).}}
        \label{fig:num-np}
    \end{minipage}%
    \hspace{0.1in}
    \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/iter-deep.pdf}
        \vspace{-0.1in}
        \figcaption{\textbf{Comparison between Single-layer Iteration \textit{v.s.} Deep Networks.}}
        \label{fig:iter-deep}
    \end{minipage}
    \hfill
    \begin{minipage}{0.35\linewidth}
        \input{tab-tex/ablation}
    \end{minipage}
\end{table*}

==> comp-tex/node-large+distri.tex <==
\begin{figure*}
    \begin{minipage}{0.58\linewidth}
        \input{tab-tex/node-large}
    \end{minipage}
    \hfill
    \begin{minipage}{0.4\linewidth}
        \centering
        % \subfigure[0]{
        %       \begin{minipage}[t]{0.33\linewidth}
        %       \centering
        %       \includegraphics[width=\textwidth]{fig/distribution/000-0.pdf}
        %       \end{minipage}}
        \vspace{-0.3in}
         \subfigure[20]{
              \begin{minipage}[t]{0.48\linewidth}
              \centering
              \includegraphics[width=\textwidth]{fig/distribution/020-0.pdf}
              \end{minipage}}
        \hspace{-0.1in}
         % \subfigure[50]{
         %      \begin{minipage}[t]{0.24\linewidth}
         %      \centering
         %      \includegraphics[width=\textwidth]{fig/distribution/050-0.pdf}
         %      \end{minipage}}
        % \hspace{-0.1in}
         % \subfigure[100]{
         %      \begin{minipage}[t]{0.24\linewidth}
         %      \centering
         %      \includegraphics[width=\textwidth]{fig/distribution/100-0.pdf}
         %      \end{minipage}}
         \subfigure[500]{
              \begin{minipage}[t]{0.48\linewidth}
              \centering
              \includegraphics[width=\textwidth]{fig/distribution/500-0.pdf}
              \end{minipage}}
        \caption{\textbf{Distribution of Embedded Nodes.} The t-sne~\cite{t-SNE} results under different training epochs are compared. \textbf{\textcolor[RGB]{22,17,139}{0}, \textcolor[RGB]{83,2,163}{1}, \textcolor[RGB]{139,10,165}{2}, \textcolor[RGB]{184,50,137}{3}, \textcolor[RGB]{219,92,104}{4}, \textcolor[RGB]{244,136,74}{5}, \textcolor[RGB]{254,189,42}{6}} denote graph nodes with different labels. \textbf{\textcolor[RGB]{197,198,199}{$\bigtriangleup$}} denotes pseudo nodes. \textbf{\textcolor[RGB]{76,255,164}{$\star$}} denotes class nodes.}
        \label{fig:distribution}
    \end{minipage}
\end{figure*}

==> comp-tex/np+iter-deep+disp.tex <==
\begin{table*}
    \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/num pnode.pdf}
        \vspace{-0.1in}
        \figcaption{\textbf{Ablation on the number of pseudo nodes\\($n_p$).}}
        \label{fig:num-np}
    \end{minipage}
    \hfill
    \begin{minipage}{0.3\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/iter-deep.pdf}
        \vspace{-0.2in}
        \figcaption{\textbf{Comparison between single shared recurrent layer and multiple recurrent layers.}}
        \label{fig:iter-deep}
    \end{minipage}
    \hfill
    % \begin{minipage}{0.3\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{fig/amz-ratings-displacement.pdf}
    %     \vspace{-0.2in}
    %     \figcaption{\textbf{Displacement Comparison on Amazon-ratings between Single Shared Parameter Layer and Multiple Parameter Layers.}}
    %     \label{fig:disp}
    % \end{minipage}
    \begin{minipage}{0.36\linewidth}
        \input{tab-tex/ablation}
    \end{minipage}
\vskip -0.1in
\end{table*}

==> fig-tex/analysis-mp.tex <==
\begin{wrapfigure}{r}{0.42\linewidth}
\vskip -0.2in
% \begin{figure}[htb]
\centering
\subfigure[$\mathrb{E}^{\texttt{np}}$]{
      \begin{minipage}[t]{0.83\linewidth}
      \centering
      \includegraphics[width=\textwidth]{fig/matrix/labeled-1-0.pdf}
      \end{minipage}}
 \subfigure[$\mathrb{E}^{\texttt{pn}}$]{
      \begin{minipage}[t]{0.83\linewidth}
      \centering
      \includegraphics[width=\textwidth]{fig/matrix/labeled-1-1.pdf}
      \end{minipage}}
\caption{\textbf{Message passing analysis.} The proximities between sampled graph nodes and pseudo nodes are depicted in the center of each sub-figure, where \textcolor[RGB]{0,96,51}{darker green} indicates higher proximity and \textcolor[RGB]{81,179,101}{brighter green} indicates lower proximity. The distribution on the top/right of each sub-figure denotes the sum of proximity for each graph/pseudo node. Graph/pseudo nodes are ranked based on the sum of proximity.}
\label{fig:mp}
% \end{figure}
\end{wrapfigure}

==> fig-tex/analysis-smoo.tex <==
% \begin{wrapfigure}{r}{0.4\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{fig/over-smoothing.pdf}
\vspace{-0.1in}
\figcaption{\textbf{Effectiveness Study on Over-smoothing.}}
\label{fig:smoothing}
% \end{wrapfigure}

==> fig-tex/analysis-squa.tex <==
% \begin{wrapfigure}{r}{0.4\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{fig/over-squashing.pdf}
\vspace{-0.1in}
\figcaption{\textbf{Effectiveness Study on Over-squashing.}}
\label{fig:squashing}
% \end{wrapfigure}

==> tab-tex/expressiveness.tex <==
\begin{table}[t]
% \vskip -0.1in
\caption{\textbf{Expressiveness Analysis on Subgraph Counting (measured by mean absolute error).}}
\label{tab:expressiveness}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc} 
\toprule
             & \multicolumn{1}{l}{Cycle5,v$\downarrow$} & \multicolumn{1}{l}{Cycle6,v$\downarrow$} & \multicolumn{1}{l}{Chordal4,v$\downarrow$} & \multicolumn{1}{l}{Chordal5,v$\downarrow$}  \\ 
\midrule
MPNN         & 0.30                         & 0.21                         & 0.32                           & 0.24                            \\
Subgraph GNN & 0.09                         & 0.08                         & 0.05                           & 0.07                            \\
Local 2-GNN  & 0.01                         & 0.02                         & 0.00                           & 0.02                            \\
Local 2-FGNN & 0.01                         & 0.02                         & 0.00                           & 0.01                            \\
\textbf{\nsqure~(Ours)}        & 0.03                         & 0.02                         & 0.07                           & 0.05                            \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vspace{-0.3in}
\end{table}

==> tab-tex/graph.tex <==
% \begin{table*}
% \begin{floatrow}
% \capbtabbox{
% \resizebox{0.6\textwidth}{!}{
% \input{tab-tex/graph small}
% }}{
% \caption{\textbf{Graph Classification Results on Small-scale Benchmarks (measured by accuracy: \%).}\TODO{substitute +!!!}}
% \label{tab:graph-small}
% }
% \hspace{-0.2in}
% \capbtabbox{
% \resizebox{0.35\textwidth}{!}{
% \input{tab-tex/graph large}
% }}{
% \vspace{0.5in}
% \caption{\textbf{Graph Classification Results on Large-scale Benchmark OGB-Molpcba (measured by average precision: \%).}\TODO{substitute +!!!}}
% \label{tab:graph-large}
% }
% \end{floatrow}
% \end{table*}
  
\begin{table*}
    \begin{minipage}{0.65\linewidth}
        \tabcaption{\textbf{Graph classification results on small-scale benchmarks (measured by accuracy: \%).}}
        \label{tab:graph-small}
        \centering
        \resizebox{\textwidth}{!}{
        \input{tab-tex/graph-small}}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.38\linewidth}
        \tabcaption{\textbf{Graph classification results on large-scale benchmark OGB-molpcba.}}
        \label{tab:graph-large}
        % \vspace{1em}
        \centering
        \resizebox{\textwidth}{!}{
        \input{tab-tex/graph-large}}
    \end{minipage}
\end{table*}

==> tab-tex/node-small.tex <==
\begin{table*}
    \tabcaption{\textbf{Node classification results on small-scale graphs (measured by ROC-AUC except accuracy for amazon-ratings: \%).} $\dagger$ denotes our reproduced results.}
    \label{tab:node-small}
    % \vskip -0.1in
    \subtable[Heteropilic Graphs\label{tab:hetero-node-small}]{
        % \tabcaption{\textbf{Node Classification Results on Small-scale Heterophilic Graphs (measured by ROC-AUC except accuracy for amazon-ratings: \%).} $\dagger$ denotes our reproduced results.}
        \centering
        \resizebox{0.5\textwidth}{!}{
        \input{tab-tex/hetero-node-small}}
    }%
    \subtable[Homophilic Graphs\label{tab:homo-node-small}]{
        \centering
        \resizebox{0.54\textwidth}{!}{
        \input{tab-tex/homo-node-small}}
    }
\end{table*}
  
% \begin{table*}
%     \begin{minipage}{0.48\linewidth}
%         \tabcaption{\textbf{Node Classification Results on Small-scale Heterophilic Graphs (measured by ROC-AUC except accuracy for amazon-ratings: \%).} $\dagger$ denotes our reproduced results.}
%         \label{tab:hetero-node-small}
%         \centering
%         \resizebox{\textwidth}{!}{
%         \input{tab-tex/hetero-node-small}}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{0.48\linewidth}
%         \tabcaption{\textbf{Node Classification Results on Small-scale Homophilic Graphs (measured by accuracy: \%).}}
%         \label{tab:homo-node-small}
%         \centering
%         \resizebox{\textwidth}{!}{
%         \input{tab-tex/homo-node-small}}
%     \end{minipage}
% \end{table*}
